Exclusion and Verification of Remote Nuclear Reactors with a 1-Kiloton Gd-Doped Water Detector

To date, antineutrino experiments built for the purpose of demonstrating a nonproliferation capability have typically employed organic scintillators, were situated as close to the core as possible -typically a few meters to tens of meters distant and have not exceeded a few tons in size. One problem with this approach is that proximity to the reactor core require accommodation by the host facility. Water Cherenkov detectors located offsite, at distances of a few kilometers or greater, may facilitate non-intrusive monitoring and verification of reactor activities over a large area. As the standoff distance increases, the detector target mass must scale accordingly. This article quantifies the degree to which a kiloton-scale gadolinium-doped water-Cherenkov detector can exclude the existence of undeclared reactors within a specified distance, and remotely detect the presence of a hidden reactor in the presence of declared reactors, by verifying the operational power and standoff distance using a Feldman-Cousins based likelihood analysis. A 1-kton scale (fiducial) water Cherenkov detector can exclude gigawatt-scale nuclear reactors up to tens of kilometers within a year. When attempting to identify the specific range and power of a reactor, the detector energy resolution was not sufficient to delineate between the two.

==> Author_List.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
%WATCHMAN
%%%%%%%%%%%%%%%%%%%%%%%%


%\author{O. A.  Akindele}\NCSDLLNL
\author{T. Anderson}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
%\author{M. Askins}	
%\affiliation{University of California at Berkeley, Berkeley,  California 94720,  USA} 
\author{Z. Bagdasarian}	
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA} 
\author{A. Baldoni}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{A. Barna}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{T. Benson}	
\affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{M. Bergevin}	
\NCSDLLNL
\author{A. Bernstein}	
\NCSDLLNL
%\author{B. Birrittella}	
%\affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{S. Bogetic}	
\NCSDLLNL
\author{J. Boissevain}	
\affiliation{University of Pennsylvania,  Philadelphia,  Pennsylvania 19104,  USA} 
\author{J. Borusinki}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{S. Boyd}	
\affiliation{University of Warwick, Coventry, CV4 7AL, UK} 
\author{T. Brooks}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
%\author{M. Budsworth}	
%\affiliation{Atomic Weapons Establishment,  Aldermaston,  Reading RG7 4PR, UK} 
\author{J. Burns}	
\affiliation{Atomic Weapons Establishment,  Aldermaston,  Reading RG7 4PR, UK} 
\author{M. Calle}	
\affiliation{Atomic Weapons Establishment,  Aldermaston,  Reading RG7 4PR, UK} 
\author{C. Camilo}\BNL	
\BNL
\author{A. Carroll}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{J. Coleman}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{R. Collins}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{C. Connor}	
\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{D. Cowen}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{B. Crow}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{J. Curry}	
\NCSDLLNL
\author{F. Dalnoki-Veress}	
\affiliation{Middlebury Institute of International Studies at Monterey, Monterey, California 93940, USA}
\affiliation{James Martin Center for Nonproliferation Studies, Monterey, California 93940, USA}\author{D. Danielson}	
\affiliation{University of Chicago, Chicago, IL 60637, USA} 
\author{S. Dazeley}	
\NCSDLLNL
\author{M. Diwan}	
\BNL
\author{S. Dixon}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
%\author{L. Drakopoulou}	
%\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{A. Druetzler}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
%\author{J. Duron}	
%\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{S. Dye}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{S. Fargher}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{A. Fienberg}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{V. Fischer}	
\affiliation{Department of Physics, University of California at Davis, Davis, California 95616, USA} 
\author{R. Foster}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{K. Frankiewicz}	
\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{T. Gamble}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
%\author{D. Gooding}	
%\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{S. Gokhale}	
\BNL
%\author{C. Grant}	
%\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{R. Gregorio}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{J. Gribble}	
\affiliation{Atomic Weapons Establishment,  Aldermaston,  Reading RG7 4PR, UK} 
\author{J. Griskevich}	
\affiliation{University of California at Irvine,  Irvine,  California 92697,  USA} 
\author{D. Hadley}	
\affiliation{University of Warwick, Coventry, CV4 7AL, UK} 
\author{J. He}	
\affiliation{Department of Physics, University of California at Davis, Davis, California 95616, USA} 
\author{K. Healey}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{J. Hecla}	
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA} 
\author{G. Holt}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{C. Jabbari}	
\affiliation{Middlebury Institute of International Studies at Monterey / James Martin Center for Nonproliferation Studies} 
\author{K. Jewkes}	
\affiliation{University of Warwick, Coventry, CV4 7AL, UK} 
\author{I. Jovanovic}	
\affiliation{University of Michigan,  Ann Arbor,  Michigan 48109,  USA} 
\author{R. Kaiser}	
\affiliation{University of Glasgow, Glasgow, G12 8QQ, Scotland,} 
\author{M. Keenan}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{P. Keener}	
\affiliation{University of Pennsylvania,  Philadelphia,  Pennsylvania 19104,  USA} 
\author{E. Kneale}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{V. Kudryavtsev}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{P. Kunkle}	
\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{J. Learned}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{V. Li}\NCSDLLNL
\author{P. Litchfield}	
\affiliation{University of Glasgow, Glasgow, G12 8QQ, Scotland,} 
\author{X. Ran Liu}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
%\author{G. Lynch}	
%\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
%\author{M. Malek}	
%\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{J. Maricic}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{P. Marr-Laundrie}	
\affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{B. Masic}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{C. Mauger}	
\affiliation{University of Pennsylvania,  Philadelphia,  Pennsylvania 19104,  USA} 
%\author{N. McCauley}	
%\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{C. Metelko}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{R. Mills}	
\affiliation{National Nuclear Laboratory (affiliated with University  of  Liverpool,  Liverpool  L69  3BX,  UK)} 
\author{A. Mitra}	
\affiliation{University of Warwick, Coventry, CV4 7AL, UK} 
\author{F. Muheim}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{A. Mullen}	
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA} 
\author{A. Murphy}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{M. Needham}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{E. Neights}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{K. Nishimura}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{K. Ogren}	
\affiliation{University of Michigan,  Ann Arbor,  Michigan 48109,  USA} 
\author{G. Orebi Gann}	
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA} 
\author{L. Oxborough}	
\affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{S. Paling}	
\affiliation{Boulby Underground Laboratory, Loftus, Saltburn-by-the-Sea, Cleveland TS13 4UZ, UK} 
\author{A. Papatyi}	
\affiliation{Pacific Northwest National Laboratory, Richland, WA 99352, USA } 
\author{B. Paulos}	
\affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{T. Pershing}	
\affiliation{Department of Physics, University of California at Davis, Davis, California 95616, USA} 
\author{L. Pickard}	
\affiliation{Department of Physics, University of California at Davis, Davis, California 95616, USA} 
\author{S. Quillin}	
\affiliation{Atomic Weapons Establishment,  Aldermaston,  Reading RG7 4PR, UK} 
\author{R. Resoro}	
\BNL
\author{B. Richards}	
\affiliation{University of Warwick, Coventry, CV4 7AL, UK} 
\author{L. Sabarots}	
\affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{A. Scarff}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{Yan-Jie Schnellbach}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{P. Scovell}	
\affiliation{Boulby Underground Laboratory, Loftus, Saltburn-by-the-Sea, Cleveland TS13 4UZ, UK} 
\author{B. Seitz}	
\affiliation{University of Glasgow, Glasgow, G12 8QQ, Scotland,} 
%\author{O. Shea}	
%\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{V. Shebalin}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
%\author{G. Smith}	
%\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{M. Smy}	
\affiliation{University of California at Irvine,  Irvine,  California 92697,  USA} 
\author{H. Song}	
\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{N. Spooner}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
%\author{C. Stanton}	
%\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{O. Stone}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{F. Sutanto}	
\affiliation{University of Michigan,  Ann Arbor,  Michigan 48109,  USA} 
\author{R. Svoboda}	
\affiliation{Department of Physics, University of California at Davis, Davis, California 95616, USA} 
\author{S. Szoldos}	
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA} 
\author{L. Thompson}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{F. Thomson}	
\affiliation{University of Glasgow, Glasgow, G12 8QQ, Scotland,} 
\author{C. Toth}	
\affiliation{Boulby Underground Laboratory, Loftus, Saltburn-by-the-Sea, Cleveland TS13 4UZ, UK} 
\author{M. Vagins}	
\affiliation{University of California at Irvine,  Irvine,  California 92697,  USA} 
\author{R. Van Berg}	
\affiliation{University of Pennsylvania,  Philadelphia,  Pennsylvania 19104,  USA} 
%\author{G. Varner}	
%\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{S. Ventura}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{B. Walsh}	
\BNL
%\author{J. Webster}	
%\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{M. Weiss}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{D. Westphal}\NCSDLLNL
\author{M. Wetstein}	
\affiliation{Iowa  State  University,  Ames,  Iowa  50011,  USA} 
\author{T. Wilson}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{S. Wilson}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{S. Wolcott}	
\affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{M. Wright}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{M. Yeh}	
\BNL
\collaboration{The WATCHMAN collaboration}
\noaffiliation
